Robustness Reprogramming for Representation Learning

This work tackles an intriguing and fundamental open challenge in representation learning: Given a well-trained deep learning model, can it be reprogrammed to enhance its robustness against adversarial or noisy input perturbations without altering its parameters? To explore this, we revisit the core feature transformation mechanism in representation learning and propose a novel non-linear robust pattern matching technique as a robust alternative. Furthermore, we introduce three model reprogramming paradigms to offer flexible control of robustness under different efficiency requirements. Comprehensive experiments and ablation studies across diverse learning models ranging from basic linear model and MLPs to shallow and modern deep ConvNets demonstrate the effectiveness of our approaches. This work not only opens a promising and orthogonal direction for improving adversarial defenses in deep learning beyond existing methods but also provides new insights into designing more resilient AI systems with robust statistics.

==> section/abs.tex <==

\begin{abstract}

% \xr{emphasize what do we mean by \textbf{Robustness Reprogramming}: control the robustness without changing the parameters of any given model}


% Deep learning models achieve remarkable success through their ability to learn rich data representations. At the core of this process is the linear mapping operator, which plays a fundamental role in encoding complex data patterns. However, these linear operations are often vulnerable to adversarial perturbations and noisy inputs. In this work, we propose a novel robustness reprogramming method to enhance the resilience of linear operations within any given model. Our comprehensive experiments demonstrate the superior robustness of our proposed method across three paradigms, and ablation studies further provide insightful understanding into the mechanisms behind its effectiveness.

% \xr{should think about a good name for our method.}


This work tackles an intriguing and fundamental open challenge in representation learning: Given a well-trained deep learning model, can it be reprogrammed to enhance its robustness against adversarial or noisy input perturbations without altering its parameters?
To explore this, we revisit the core feature transformation mechanism in representation learning and propose a novel non-linear robust pattern matching technique as a robust alternative. Furthermore, we introduce three model reprogramming paradigms to offer flexible control of robustness under different efficiency requirements. Comprehensive experiments and ablation studies across diverse learning models ranging from basic linear model and MLPs to shallow and modern deep ConvNets demonstrate the effectiveness 
of our approaches.
This work not only opens a promising and orthogonal direction for improving adversarial defenses in deep learning beyond existing methods but also provides new insights into designing more resilient AI systems with robust statistics. 
Our implementation is available at \href{https://anonymous.4open.science/r/NRPM-322C/}{https://anonymous.4open.science/r/NRPM-322C/}.


\end{abstract}

==> section/algorithm_v1.tex <==

\subsection{Algorithm Development}
To this end, we leverage the iterative reweighted least squares algorithm to tackle this challenging problem. 
We
first design a localized upper bound for the original objective and then optimize the upper bound with
a second-order Newton method. We also provide a rigorous theoretical loss descent guarantee.

\textbf{Localized upper bound.}
Instead of directly optimizing the original loss function $\mathcal{L}(\vz)$ in Eq.~\ref{eq:robust_estimation}, 
we optimize a convex localized upper bound at the current iteration $\vz^{(k)}$ as follows:

\begin{lemma}[Localized Upper Bound] 
\label{lemma:local_upper_bound}
Suppose the loss objective is
$\mathcal{L}(\vz)=\sum_{i=1}^{N} |\vz/N-\va_i\cdot \vx_i|^p$ ($p\leq 2$) as in Eq.~\eqref{eq:robust_estimation}. For any fixed point $\vz^{(k)}$, there exists a convex localized upper bound as:
\begin{equation}
\label{eq:upper_bound}
\hat{\mathcal{L}}(\vz)=\sum_{i=1}^N w_i^{(k)}\cdot (\va_i\vx_i-\vz/N)^2+C(\vz^{(k)}),
\end{equation}
where $w_i^{(k)}=\frac{1}{|\va_i\vx_i-\vz^{(k)}/N|^{2-p}}$.  Particularly, the constant $C(\vz^{(k)})$  guarantees the equality of $\hat{\mathcal{L}}$ and $\mathcal{L}$ at $\vz^{(k)}$, i.e., $\hat{\mathcal{L}}(\vz^{(k)})=\mathcal{L}(\vz^{(k)})$. 

\end{lemma}

\begin{proof}
    Define  $\phi(z):=z^{\frac{p}{2}} (p\leq 2)$, which is a non-convex function, then for fixed point $z_0$, $$\phi(z)\leq\phi(z_0)+\phi^\prime(z_0)(z-z_0)=\phi^\prime(z_0)\cdot z+C(z_0)$$
where the first inequality holds with equality at $z=z_0$ and
$\phi^\prime(z_0)=\frac{p}{2}z_0^{\frac{p}{2}-1}.$


when $p=1$, $$\sqrt{z}\leq\sqrt{z_0}+\frac{1}{2\sqrt{z_0}}(z-z_0)=\frac{z}{2\sqrt{z_0}}+\frac{\sqrt{z_0}}{2}$$

By replacemnet as $z=(\va_i\vx_i-\vz/N)^2$ and $z_0=(\va_i\vx_i-\vz^{(k)}/N)^2$, then
\begin{align*}
    |\va_i\vx_i-\vz/N|&\leq \frac{p}{2}\cdot \frac{1}{|\va_i\vx_i-\vz^{(k)}/N|^{2-p}}\cdot (\va_i\vx_i-\vz/N)^2+C(|\va_i\vx_i-\vz^{(k)}/N|)\\
    &=w_i^{(k)}\cdot (\va_i\vx_i-\vz/N)^2+C(|\va_i\vx_i-\vz^{(k)}/N|),
\end{align*}








where $w_i^{(k)}=\frac{p}{2}\cdot \frac{1}{|\va_i\vx_i-\vz^{(k)}/N|^{2-p}}$ and the first inequality holds with equality at $\vz=\vz^{(k)}$.
Sum up the items on both sides with weights $\{a_j\}_{j\in[N]}$, we obtain
\begin{equation}
\label{eq:upper_bound_inequlity}
\begin{split}
\mathcal{L}(\vz)&=\sum_{i=1}^{N} |\va_i\cdot \vx_i -\vz/N| \\
&\leq \sum_{i=1}^N w_i^{(k)}\cdot (\va_i\vx_i-\vz/N)^2+\sum_{i=1}^NC(|\va_i\vx_i-\vz^{(k)}/N|) \\
&=\sum_{i=1}^N w_i^{(k)}\cdot (\va_i\vx_i-\vz/N)^2+C(\vz^{(k)})\\
&=\hat{\mathcal{L}}(\vz)
\end{split}
\end{equation}

$$\mathcal{L}(\vz,\vz_0)$$


and the equality holds at $\vz=\vz^{(k)}$:
\begin{equation}
\label{eq:local_equality}
    \hat{\mathcal{L}}(\vz^{(k)})=\mathcal{L}(\vz^{(k)}).
\end{equation}
\end{proof}


As  $C(\vz^{(k)})$ is treated as a constant during the optimization at the current step, the upper bound in Eq.~\ref{eq:upper_bound} becomes convex and can be efficiently optimized.


\textbf{Newton-IRLS iteration.} After obtaining the convex upper bound $\hat{\cL}$ in Eq.~\eqref{eq:upper_bound}, 
we can derive a concise closed-form iteration using the second-order Newton method as follows:
\begin{align}
    \vz^{(k+1)}
    &=\vz^{(k)}-\left[\nabla^2 \hat{\mathcal{L}}(\vz^{(k)})\right]^{-1}\nabla \hat{\cL}(\vz^{(k)})=N\cdot \frac{\sum_{i=1}^N  w^{(k)}_i \va_i\vx_i}{\sum_{i=1}^N  w^{(k)}_i}
    \label{eq:reweight}
\end{align}
\begin{proof}


$$\hat{\mathcal{L}}^\prime(\vz^{(k)})=\frac{1}{N}\sum_{i=1}^N w^{(k)}_i\cdot 2(\vz^{(k)}/N-\va_i\vx_i)$$

$$ \hat{\mathcal{L}}^{\prime\prime}(\vz^{(k)})=\frac{2}{N^2}\sum_{i=1}^N  w^{(k)}_i $$


\begin{align}
\vz^{(k+1)}&=\vz^{(k)}-\frac{\hat{L}^\prime(\vz^{(k)})}{ \hat{L}^{\prime\prime}(\vz^{(k)})}\\
&=\vz^{(k)}-\frac{\frac{1}{N}\sum_{i=1}^N w^{(k)}_i\cdot 2(\vz^{(k)}/N-\va_i\vx_i)}{\frac{2}{N^2}\sum_{i=1}^N  w^{(k)}_i}\\
&=N\cdot \frac{\sum_{i=1}^N  w^{(k)}_i \va_i\vx_i}{\sum_{i=1}^N  w^{(k)}_i}
\end{align}

where $w_i^{(k)}=\frac{p}{2}\cdot \frac{1}{|\va_i\vx_i-\vz^{(k)}/N|^{2-p}}.$ 
Since the constant in $w_i^{(k)}$ can be canceled in the updated formulation, we have:
$$w_i^{(k)}= \frac{1}{|\va_i\vx_i-\vz^{(k)}/N|^{2-p}}.$$


\end{proof}

Eq.~\eqref{eq:reweight} can be interpreted as a reweighted sum, in which the derived $w^{(k)}_j$ modifies the original kernel weight $\va_i$ on the input pixel $\vx_i$. 
The convergence of the Newton-IRLS algorithm  and rigorous loss descent are guaranteed by the following Theorem~\ref{thm:loss-descent}.
\begin{theorem}[Convergence guarantee]
\label{thm:loss-descent}
Suppose the loss objective $\cL(\vz)$ is defined as in Eq.~\eqref{eq:robust_estimation} and its corresponding convex localized upper bound is in Eq.~\eqref{eq:upper_bound}. Then, through the iteration in Eq.~\eqref{eq:reweight}, the following inequality holds:
    \begin{equation}
     \cL(\vz^{(k+1)})\leq\hat{\cL}(\vz^{(k+1)})\leq\hat{\cL}(\vz^{(k)})=\cL(\vz^{(k)}),
    \end{equation}
that is, optimizing upper bound $\hat{\cL}$ can guarantee the rigorous descent of $\cL$.
\end{theorem}
\begin{proof}
    Since $\vz^{(k+1)}$ is obtained from optimize the convex localized upper bound $\cL$ at $\vz^{(k)}$, then we have $\hat{\cL}(\vz^{(k+1)})\leq\hat{\cL}(\vz^{(k)})$. According to the  upper bound in Eq.~\eqref{eq:upper_bound_inequlity} and  localized equality in Eq.~\eqref{eq:local_equality}, it is not hard to get the following inequality:
    $$\cL(\vz^{(k+1)})\leq\hat{\cL}(\vz^{(k+1)})\leq\hat{\cL}(\vz^{(k)})=\cL(\vz^{(k)}).$$
    Therefore, optimizing the localized upper bound $\hat{\cL}$ can guarantee the rigorous descent of $\cL$.
\end{proof}



==> section/exp_subsection/exp_other.tex <==

\newpage
\subsection{Out-of-distribution (ood) Robustness}

Out-of-distribution robustness~\citep{li2024oodrobustbench} under distribution shift becomes even more important in recent year. 


\begin{table}[!ht]
    \centering
    \caption{CIFAR-10-C-All-Corruptions (complete)}
    \begin{tabular}{l|l|c|c|c|c|c}
    \hline
    Noise Type&Model&Level 1&Level 2&Level 3&Level 4&Level 5\\
    \toprule
        \textbf{Noise} & ~ & ~ & ~ & ~ & ~ &   \\ \hline
        gaussian\_noise & L2 & 63.62 & 43.00 & 28.23 & 23.18 & 20.10  \\ \hline
         & MCP & 68.17 & 51.73 & 38.73 & 33.85 & 30.20  \\ \hline
        impulse\_noise & L2 & 75.00 & 64.11 & 52.96 & 35.62 & 24.43  \\ \hline
         & MCP & 73.72 & 63.40 & 54.28 & 41.24 & 31.41  \\ \hline
        shot\_noise & L2 & 72.61 & 61.71 & 39.08 & 31.85 & 23.96  \\ \hline
         & MCP & 75.65 & 66.80 & 48.65 & 42.47 & 34.37  \\ \hline
        speckle\_noise&L2&72.87&56.13&48.85&36.32&27.89\\\hline
                 &MCP&74.25&61.02&54.94&44.18&35.05\\\hline
        \textbf{Blur} & ~ & ~ & ~ & ~ & ~ &   \\ \hline
        motion\_blur & L2 & 78.36 & 67.97 & 59.48 & 59.29 & 52.53  \\ \hline
        & MCP & 78.17 & 69.20 & 63.57 & 63.38 & 56.58  \\ 
        \hline
        defocus\_blur & L2 & 86.69 & 84.35 & 77.40 & 66.23 & 46.52  \\ \hline
         & MCP & 86.28 & 83.71 & 76.37 & 69.33 & 60.92  \\ \hline
        glass\_blur & L2 & 32.43 & 34.62 & 37.50 & 28.21 & 29.58  \\ \hline
         & MCP & 38.46 & 40.50 & 43.13 & 33.54 & 35.59  \\ \hline
zoom\_blur & L2 & 76.53 & 72.72 & 65.98 & 60.23 & 50.45  \\ \hline
         & MCP & 75.54 & 71.48 &  68.20 & 64.94 & 59.76  \\ \hline
         
        \textbf{Weather} & ~ & ~ & ~ & ~ & ~ &   \\ \hline
        fog & L2 & 86.41 & 84.01 & 80.32 & 74.56 & 54.70  \\ \hline
         & MCP & 86.41 & 83.91 & 80.01 & 74.40 &  57.38 \\ \hline
        snow & L2 & 77.62 & 58.34 & 66.38 & 62.95 & 54.51  \\ \hline
        & MCP & 76.80 & 61.58 & 67.16 & 63.53 & 57.74  \\ \hline
        frost & L2 & 78.61 & 69.45 & 54.86 & 51.96 & 40.36  \\ \hline
         & MCP & 77.82 & 68.58 & 56.52 & 55.13 & 44.33  \\ \hline
\textbf{Digital} & ~ & ~ & ~ & ~ & ~ &   \\ \hline
        brightness  & L2 & 84.75 & 84.12 & 83.40 & 82.32 & 79.45 \\ \hline
         & MCP & 85.64 & 84.62 & 83.55 & 83.14 & 80.79  \\ \hline
        contrast & L2 & 83.66 & 73.52 & 61.98 & 45.23 & 24.63  \\ \hline
         & MCP & 85.78 & 77.43 & 67.91 & 52.59 & 24.23  \\ \hline
        elastic\_transform & L2 & 77.89 & 77.28 & 72.59 & 68.58 & 64.20 \\ \hline
         & MCP & 78.79 & 78.92 & 74.17 & 70.22 & 66.49  \\ \hline
        pixelate & L2 & 82.89 & 74.34 & 66.76 & 49.02 & 36.60  \\ \hline
         & MCP & 81.34 & 71.10 & 63.65 & 46.56 & 35.48  \\ \hline
        jpeg\_compression & L2 & 79.82 & 75.21 & 73.8 & 72.20 & 69.19  \\ \hline
         & MCP & 80.77 & 76.49 & 75.25 & 72.94 & 69.83  \\ \hline
    \end{tabular}
\end{table}







==> section/intro_v1.tex <==
\iffalse
\xr{some potential titles:
\begin{itemize}
    \item Reconfigurable Robust Representation Learning
    \item Programmable Robust Representation Learning
    \item Robustness Reprogramming for (Deep) Representation Learning
    \item (Deep) Representation Learning with Robustness Reprogramming
    \item Robust Representation Learning via Model Reprogramming
\end{itemize}
}
\fi

\section{Introduction}

\xr{the current story is not exciting. Please rewrite it according to our new story on robustness reprogramming. need to highlight the drawbacks of existing approaches and why robustness reprogramming is challenging. We need to write a story to show it is a big breakthrough}

% In response to the susceptibility of neural networks to adversarial examples~\cite{szegedy2013intriguing,biggio2013evasion},
% there has been significant interest recently in constructing defenses to increase the robustness of neural networks. While many methods attempt to defend the model from the various perspective, adversarial training-based methods~\cite{madry2017towards} have exhited great robustness in various domains. Particularly, adversarial training have dominated robust deep learning in computer vision in many years. Therefore, it is imperitive to make a breakthrough in this field to exceed the robustness limit of adversarial training.

% As we know, adversarial training enhance the robustness of models  by generating the adversairial examples and make the models learn from the worst-case scenario, as to make the mdoels more resilient to adversarial perturbations. There are a series of advanced adversarial training method~\cite{} which try to either further improve the tradeoff of the natural and robust peformance or make the training process more efficent, but all this methods are orthogonal to the model architectures. 

% Although there exists some works focus on some robust architectures,  but most of them have been  either validated false of security or rely on some empirical techques. Most of them are quite underperform the adversarial training. Moreover, to the best of our knowledge, no one have investigated how to fullfill the pontential adverarial training though a fundamental robust architecture design. 

% To address this research gap, we propose to design a innovative and universaril  architecture to enhance the robsustness of existing deep learning models. We know that most of the deep learning models are feature learning module which share similar basic characteristics that the output is usually the linear comibination of the inputs feature.
% While the linear combination is often sensitive to change the input values especially when adversarial perturbations may introduce some outlying values which disburt the natural feature, we leverage the robust statistic theory to motivate the architecture design. Our novel design can significantly improve over any given backbones, and can be combined with existing adversarial training methods to further improve the robustness.


Recent studies have underscored the vulnerability of neural networks to adversarial attacks, prompting a surge of interest in developing robust defenses~\cite{szegedy2013intriguing,biggio2013evasion}. Among various defensive strategies, adversarial training has proven particularly effective, consistently setting benchmarks in robust deep learning, especially within the realm of computer vision~\cite{madry2017towards}. This dominance underscores the critical need for innovative breakthroughs that push beyond the current limits of adversarial robustness.

Adversarial training bolsters model resilience by training on adversarial examples, thus preparing the model to withstand worst-case scenarios. While recent advancements have sought to optimize the trade-off between natural performance and robustness or to streamline the training process, these improvements generally do not alter the underlying model architecture~\cite{}.
Although some research has explored robust architectural designs, these efforts often fall short in security validations or depend heavily on empirical techniques, failing to outperform conventional adversarial training approaches. Remarkably, there is a lack of investigation into harnessing the full potential of adversarial training through fundamental architectural innovations.

In response to this research gap, we propose a novel and universally applicable architecture designed to enhance the robustness of deep learning models fundamentally. Recognizing that most deep learning models function as feature-learning modules where outputs typically result from linear combinations of input features, we identify a vulnerability: linear combinations are particularly susceptible to input perturbations, which can drastically distort output features in the presence of adversarial attacks. To mitigate this, we incorporate principles from robust statistics into our architectural design. This approach not only improves upon existing model backbones but also complements and enhances the effectiveness of adversarial training methodologies, offering a significant advancement in model robustness.


Our contributions can be summarized as follows:
\begin{itemize}[left=0.0em]
    \item 
\end{itemize}

==> section/intro_v2.tex <==
\iffalse
\xr{some potential titles:
\begin{itemize}
    \item Reconfigurable Robust Representation Learning
    \item Programmable Robust Representation Learning
    \item Robustness Reprogramming for (Deep) Representation Learning
    \item (Deep) Representation Learning with Robustness Reprogramming
    \item Robust Representation Learning via Model Reprogramming
\end{itemize}
}
\fi

\section{Introduction}



In recent years, the vulnerability of neural networks to adversarial examples~\citep{szegedy2013intriguing,biggio2013evasion} has emerged as a critical obstacle to the deployment of AI in security-sensitive applications. Various defense mechanisms have been introduced to counteract this weakness~\citep{xu2020adversarial}, among them, adversarial training~\citep{madry2017towards} has 
% established itself as the reigning champion,
consistently set the bar for robustness in deep learning, particularly in the domain of computer vision. This dominance also reveals the stagnation of innovation in adversarial robustness, which underscores the critical need for innovative breakthroughs that push the boundaries of what is currently possible and redefine the frontier of robust neural networks.

\zc{don't mention one specific one, just summarize the existing techniques, in high-level, avoid mentioning the obfuscticated gradient}

  


% The limitations of present approaches highlight the urgent need for a breakthrough. Our research aims to transcend these limitations by addressing both the architectural design of neural networks and the optimization of their parameters. The era of incremental improvements must give way to bold, transformative advances.


\zc{this part can be put in related works} The research for robust neural networks has traditionally revolved around two primary avenues: refining model architectures, $f$, and optimizing their parameters, $\vW$. On the one hand, efforts to build robust architectures often rely on obfuscated gradients~\citep{athalye2018obfuscated} or detection mechanisms, which give a false sense of security and are easily subject to adaptive attacks. These methods, while initially promising, are still vulnerable when faced with more sophisticated adversarial techniques. Additionally, designing new architectures demands significant resources, as models must frequently be trained from scratch to fully exploit their potential.

\zc{start to computation cost, training cost, hard to control the trade-off of clean and robust, not general}

On the other hand, parameter optimization techniques like adversarial training~\citep{madry2017towards} and stability learning~\citep{zheng2016improving,cisse2017parseval} have demonstrated effectiveness but tend to overlook the latent robustness that could be harnessed from the model’s architecture itself. Adversarial training, for instance, integrates adversarial examples into the training process but is heavily reliant on attack algorithms to generate meaningful perturbations, and often falls into severe overfitting pitfall. Stability learning, which aims to regulate properties like the Lipschitz constant or influence function, only adjusts parameters to improve robustness without sufficiently exploring the inherent robustness capabilities that certain architectures may possess.

In response to these research gaps, we propose a groundbreaking approach: \textit{Robustness Reprogramming}. Our strategy seeks to unlock the full potential of both the model architecture $f$ and its parameters $\vW$, offering a comprehensive solution that harmonizes architectural design with parameter optimization. This novel framework promises to redefine the landscape of robust deep learning, opening new pathways to resilience in the face of adversarial threats.

Our contributions can be summarized as follows:
\begin{itemize}[left=0.0em]
    \item 
\end{itemize}


==> section/method_v1.tex <==
\newpage
\section{RosNets}

\xr{This section can talk about \textbf{representation learning} and our technique. We can have next section to introduce robustness reprogramming}







\textbf{Notation.} 
We denote the input embedding local patch as $\vX\in\mathbb{R}^{K \times K \times D_1}$, the output embedding as $\vZ\in \mathbb{R}^{D_2}$, the
learnable kernel as $\vK\in\mathbb{R}^{ K \times K \times D_1\times D_2}$, where $K, D_1,D_2$ are kernel size, input dimension, and output dimension, respectively.
For simplicity, we consider output dimension $D_2$ as $1$, then we have $\vK\in \mathbb{R}^{K\times K\times D_1}$ and  $\vZ\in \mathbb{R}$.
When $K=1$, the convolution is reduced to the MLP case. 

It is well-known that median estimation is less sensitive to outliers and more robust than mean estimation. From an optimization perspective, if we consider the unified $\ell_p$-estimation as:
$
\arg\min_\vz \sum_{i=1}^N |\vz - \vx_i|^p,
$
where $\{\vx_i\}_{i=1}^N$ are the data points to be fitted and $\vz$ is the estimation over them. Hence, it is not difficult to see that the mean corresponds to $\ell_2$-estimation, while the median corresponds to $\ell_1$-estimation.

\zc{provide a table to compare the L2 and L1 models like KAN}




% \subsection{Convolution/MLPs as $\ell_2$-estimator}
\subsection{A New Perspective of Representation Learning}

First, we introduce a novel perspective to express the basic linear operator in Convolution/MLPs as $\ell_2$-estimator. Specifically, each output embedding is represented as a weighted sum of the local patch and the kernel weights:
\[
\vZ=\sum_{i=1}^{N}\vK_i\cdot\vX_i, \text{where } N=K*K*D_1.
\]
This weighted sum can be interpreted as the optimal solution to the following $\ell_2$-error minimization problem:
\[
\arg\min_\vZ\mathcal{L}(\vZ)= \sum_{i=1}^{N}\left(\frac{\vZ}{N}-\vK_i\cdot\vX_i\right)^2,
\]
where the first-order optimality condition
$
\frac{\partial \mathcal{L} }{\partial \vZ}=\frac{2}{N}\sum_{i=1}^N\left(\frac{\vZ}{N}-\vK_i\cdot \vX_i\right) =0
$
leads to the solution:
$
\vZ=\sum_{i=1}^N\vK_i\cdot \vX_i.
$



% \input{section/method-rosnet_v1}
\input{section/method-rosnet_v2}


\subsection{RosNets: Robust Convolution/MLP Layer}
In previous section, we formulate the pixel-wise Newton-IRLS approach for notation simplicity. However, it is not trivial to implement such theory into practice in convolution and MLPs layer. In this section, we will present the detailed implementation or techniques for each case.

\subsubsection{RosMLP}
In MLPs, the model reduces to the case of $K=1$. Denote the input as $\vX\in\mathbb{R}^{D_1}$, the output embedding as $\vZ\in \mathbb{R}^{D_2}$, the
learnable weight as $\vK\in\mathbb{R}^{ D_1\times D_2}$, 


\begin{algorithm}[H]
\caption{RosMLPs}
\label{alg:irls}
\begin{small}
\begin{minted}[escapeinside=||,mathescape=true,linenos=true, numbersep=-3pt, framesep=3mm]{Python}
 def RosMLP(X, K, eps = 1e-3):
     KX = X.unsqueeze(-1) * K
     Z = torch.matmul(X, K) # Initialization as $\ell_2$-estimation
     For _ in range(T):
        D = torch.abs(KX - Z/N) # Distance
        W = 1/(D + eps)
        W = normalize(W * A, p=1, dim=0) 
        Z = N*(W*KX).sum(dim=0) # Update
\end{minted}
\end{small}
\end{algorithm}


\subsubsection{RosConv}
\label{sec:rosconv}
\textbf{Unfolding.}
To apply robust estimation over each patch, we must first unfold the convolution into multiple patches and process them individually. While it's possible to use a for loop to extract patches across the channels, height, and width, this approach introduces redundancy and increases computational complexity. Instead, we can leverage PyTorch's \texttt{torch.nn.functional.unfold} function to streamline and accelerate both the unfolding and computation process.

\textbf{Learnable combination of $\ell_2$ and $\ell_1$-estimation.} 
While $\ell_1$-estimation enhances model robustness, we observe that it can lead to a decline in clean accuracy, especially as models deepen. This may be due to the growing estimation error between $\ell_2$ and $\ell_1$-estimation across layers. To leverage the strengths of both $\ell_1$ and $\ell_2$-based models, we propose combining these two embeddings with a learnable weight $\beta$:
$$\vZ^{(0)}=\vZ_{\ell_2}$$
$$\vZ^{(k+1)}=N\cdot \frac{\sum_{i=1}^N  w^{(k)}_i \vK_i\vX_i}{\sum_{i=1}^N  w^{(k)}_i},  \text{where }  w_i^{(k)}=\frac{\rho^\prime(|\vK_i\vX_i-\vZ^{(k)}/N|)}{2|\vK_i\vX_i-\vZ^{(k)}/N|}, k=0,...,K-1$$


$$\vZ = \sigmoid(\beta)\cdot\vZ_{\ell_2}+(1-\sigmoid(\beta))\cdot \vZ^{(K)}$$
With learnable $\beta$ in adversarial training, our models can automatically select the optimal combination to improve the clean and robust performance.




==> section/method_v2.tex <==
\newpage
\section{Robust Nonlinear Feature Pattern Matching}


\xr{it is better to provide a short motivation}

In this section, we begin by exploring the vulnerability of current deep learning models from the perspective of representation learning, and subsequently introduce a novel robust feature pattern matching  in Section~\ref{sec:represenation_learning}. Following this, we develop an IRLS algorithm, which is unrolled into robust layers, as detailed in Section~\ref{sec:algo_develop}.
Lastly, we present a theoretical analysis of the robustness of this architecture in Section~\ref{sec:theoretical_robustness_analysis}.


\xr{a high-level suggestion is to pay attention to the logic and transition between sections, subsections, paragraphs, and even sentences. Make the logic and transition smooth, then it is easy for the reviewers to follow and understand}

\textbf{Notation.} 
Let the input features of one instance be represented as $\rvx = \left(\rvx_1, \dots, \rvx_D\right)^\top \in \mathbb{R}^D$, and the parameter vector as $\rva = \left(\rva_1, \dots, \rva_D\right)^\top \in \mathbb{R}^D$, where $D$ denotes the dimensionality of the input. For simplicity, we derive our method in the case where the output is one-dimensional, i.e., $\rvz \in \mathbb{R}$.



% \textbf{Notation.} 
% We denote the input embedding local patch as $\rvx\in\mathbb{R}^{K \times K \times D_1}$, the output embedding as $\rvz\in \mathbb{R}^{D_2}$, the
% learnable kernel as $\rva\in\mathbb{R}^{ K \times K \times D_1\times D_2}$, where $K, D_1,D_2$ are kernel size, input dimension, and output dimension, respectively.
% For simplicity, we consider output dimension $D_2$ as $1$, then we have $\rva\in \mathbb{R}^{K\times K\times D_1}$ and  $\rvz\in \mathbb{R}$.
% When $K=1$, the convolution is reduced to the MLP case. 

% \textbf{Notation.} 
% We denote the input as $\rvx=(\rvx_1,...,\rvx_N)^\top\in\mathbb{R}^{D}$, the output  as $\rvz\in \mathbb{R}$, the
% weight/parameter as $\rva =(\rva_1,...,\rva_N)^\top\in\mathbb{R}^{ N}$, where $N$ is the number of the input points.



% \subsection{Convolution/MLPs as $\ell_2$-estimator}
\subsection{A New Perspective of Representation Learning}
\label{sec:represenation_learning}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/model_comparison.png}
    \caption{Vanilla Architecture ($\ell_2$-model) vs. Robust Architecture ($\ell_1$-model). 
    \xr{this figure might take too much space. We can make more space for experiments. May need to shrink the space a little bit}}
    \label{fig:model_comparison}
\end{figure}

Fundamentally, deep neural networks (DNNs) inherently function as representation learning modules by transforming raw data into progressively more complex embeddings~\citep{liu2015representation}. The linear feature transformation, $\rvz=\rva^\top\rvx=\sum_{d=1}^D\rva_d\cdot\rvx_d$, is essentially the building block of deep learning models to disentangle key explanatory factors and capture particular feature patterns of interest. Specifically, a key explanatory factor $\rvx_d$ may be highly correlated with and matched by a large $\rva_d$.


Despite the impressive capability of linear operator in enhancing the representation learning of DNNs, the vanilla deep learning models have been validated highly vulnerable~\citep{szegedy2013intriguing,biggio2013evasion}. Existing approaches including robust training and regularization techniques~\citep{madry2017towards, cisse2017parseval,zheng2016improving} aim to improve the robustness of feature transformations by reshaping the parameter $\rva$ with particular properties. However, these methods  inevitably alter the feature matching behaviors, lead to clean performance degradation without necessarily achieving improved robustness. 





 % The success of deep learning models highly relies on  representation learning~\citep{liu2015representation},
 % that captures and represents the core data structures~\citep{liu2015representation}.  This stems from the fact that various representations possess the ability to  reveal  the underlying factors of variation within the data. 
 % Among the numerous techniques employed in representation learning, linear mapping stand out as both fundamental and essential operator for capturing these patterns, offering a straightforward yet powerful method to disentangle key explanatory factors. Its simplicity and effectiveness make them foundational operators in representation learning, providing a solid base for more complex models to build upon.  \xr{this description can be improved. We need to talk about the key point of representation learning}

 % Indeed, the linear feature transformations are commonly employed within the modules of various deep learning models. For instance, the Multi-layer Perceptron (MLP) fundamentally consists of a sequence of stacked linear layers, convolution operations perform a linear feature mapping over the kernel and the local patch, and the attention mechanism~\citep{vaswani2017attention} is essentially a linear transformations over the context token vectors.
 % % , and graph message aggregation fundamentally represents a linear combination of neighborhoods' information. 
 % \xr{do not need to talk about aggregation, focus on linear feature transformation}

  
 
% Despite the widespread applications and influence of linear operations in deep learning, these fundamental operations are highly vulnerable to adversarial attacks, which pose significant challenges to safeguarding the models. While many existing effective defense strategies focus on optimizing parameters or weights to enhance robustness, they often overlook the potential to explore deeper structural changes within the  mapping itself. This motivates the need to rethink the underlying reasons behind the vulnerability of the basic linear structure of representation learning, aiming for more resilient and adaptive architectures.



% Hence, we may formally unify the linear mapping as a weighted sum of the input and the weight:
% \[
% \rvz = \rva^\top\rvx = \sum_{d=1}^{D} \rva_d \cdot \rvx_d
% \]

% This weighted sum can be interpreted as the optimal solution to the following ordinary least squares (OLS) problem:
% \[
% \arg\min_\rvz \mathcal{L}(\rvz) = \sum_{d=1}^{D} \left(\frac{\rvz}{D} - \rva_d \cdot \rvx_d\right)^2,
% \]
% where the first-order optimality condition,
% \(
% \frac{\partial \mathcal{L}}{\partial \rvz} = \frac{2}{D} \sum_{d=1}^D \left(\frac{\rvz}{D} - \rva_d \cdot \rvx_d\right) = 0,
% \)
% leads to the solution:
% \(
% \rvz = \sum_{d=1}^D \rva_d \cdot \rvx_d.
% \)

% Since OLS estimation is more sensitive to the outlying value,  we tend to choose an alternative
% least absolute deviation (LAD) estimation 
% as:
% \begin{equation}
%     \mathcal{L}(\rvz) = \sum_{d=1}^{D} \left|\frac{\rvz}{D} - \rva_d \cdot \rvx_d\right|,
%     \label{eq:robust_estimation}
% \end{equation}
% Unfortunately, the proposed robust LAD estimator is both non-convex and non-smooth, posing a challenge for the design of efficient algorithms to be unrolled as layers in the neural network.



% \xr{here, the reviewers must get confused about the notations. $\{\rvx_d\}$ seems like a dataset with many input data points. We need to emphasize this is instance-level, and use dimension to highlight these are different feature dimensions from the same data point}


To this end, we aim to introduce a novel perspective by exploring how to design an alternative mapping that enhances robustness while preserving feature matching behaviors.
Firstly, we may formally express the linear feature pattern matching
 as the optimal closed-form solution of the Ordinary Least Squares (OLS) problem:
\[
\min_{\rvz\in\mathbb{R}} \mathcal{L}(\rvz)= \sum_{d=1}^{D} \left(\frac{\rvz}{D} - \rva_d \cdot \rvx_d\right)^2,
\]
where the first-order optimality condition $\nabla_{\rvz}\cL=0$ yields the \(
\rvz^* = \sum_{d=1}^{D} \rva_d \cdot \rvx_d
\).
Since OLS estimation is highly sensitive to outlying values due to the quadratic penalty, an alternative robust approach is the Least Absolute Deviation (LAD) estimation:
\begin{equation}
    \min_{\rvz\in\mathbb{R}}\mathcal{L}(\rvz) = \sum_{d=1}^{D} \left|\frac{\rvz}{D} - \rva_d \cdot \rvx_d\right|.
    \label{eq:robust_estimation}
\end{equation}
By replacing the quadratic penalty with a linear alternative on the residual $\rvz/D - \rva_d \cdot \rvx_d$, the impact of outliers can be mitigated to some extent.


% \xr{here, we should explain the motivation of this LAD estimation and why we believe it is more robust}












% \textbf{Rethinking Mean \& Median from the optimization perspective.}
% It is universally acknowledged that the estimation of the median is less susceptible to outliers and exhibits greater robustness in comparison to the estimation of the mean. From the perspective of optimization, if one considers the unified \textbf{$\ell_p$-estimation} defined as:
% \[
% \arg\min_\rvz \sum_{d=1}^D |\rvz - \rvx_d|^p,
% \]
% where $\{\rvx_d\}_{d=1}^D$ represent the data points to be fitted and $\rvz$ signifies the estimation over them. Consequently, it is apparent that the mean is associated with $\ell_2$-estimation, whereas the median is associated with $\ell_1$-estimation.

% \textbf{Conventional representation learning as $\ell_2$-estimation.}
% Deep neural networks may be conceptualized as representation learning models that typically encode information into  a different subspace.
% Given that undefended neural networks have been empirically validated to be highly susceptible to adversarial examples \citep{szegedy2013intriguing,biggio2013evasion}, we seek to rethink deep representation learning from an innovative perspective to reveal the fundamental reasons behind this vulnerability.







\input{section/algorithm_v2}

\subsection{Theoretical Robustness Analysis}
\label{sec:theoretical_robustness_analysis} 
In the previous section, we designed a robust architecture using the IRLS algorithm, as outlined in Algorithm~\ref{alg:irls_algo}. In this section, we conduct a theoretical robustness analysis comparing the vanilla architecture with our robust design, utilizing the influence function~\citep{law1986robust}. Consider the $\ell_2$-model: $\rvz_{\ell_2} = \sum_{d=1}^D \rva_d \rvx_d$ and  $\ell_1$-model: $\rvz^{(k+1)}_{\ell_1} = N \cdot \frac{\sum_{d=1}^D w_d^{(k)} \rva_d \rvx_d}{\sum_{d=1}^D w^{(k)}_d},$ where $w^{(k)}_d = \frac{1}{|\rva_d \rvx_d - \rvz^{(k)}_{\ell_1} / N|}$ and $\rvz_{\ell_1}^{(0)} = \rvz_{\ell_2}$ for $k = 0, 1, ..., K-1$.
To simplify the notation, we consider a single-step case for our IRLS algorithm ($K=1$). Replace $\rva_d \rvx_d$ with $\rvx_d$ and represent the data distribution as $F(\rvx)=\frac{1}{D}\sum_{d=1}^D\mathbb{I}_{\{\rvx=\rvx_d\}}$. Define the transformations $\vy=T_{\ell_2}(F)=\frac{1}{D} \sum_{d=1}^D \rvx_d$ and $\rvz=T_{\ell_1}(F)=\frac{\sum_{d=1}^D w_d \rvx_d}{\sum_{d=1}^D w_d}$, where $w_d = \frac{1}{|\rvx_d - \vy|}$. 
\xr{it seems the theorem only considers the case when only one feature dimension can be attacked? If so, is it possible to make it more general? Or at least we need to justify why this is still valuable. For instance, the influence analysis implies the impact of each feature dimension on the output individually}
Then we can obtain the influence function of $\ell_2$ and $\ell_1$ model as follows:
    

\begin{theorem}[Robustness Analysis via Influence Function]
\label{thm:influence_function} 

The influence function is defined as the sensitivity of the estimate to a small contamination at \( \rvx_0 \):
\[
IF(\rvx_0; T,F) = \lim_{\epsilon \to 0} \frac{T(F_\epsilon) - T(F)}{\epsilon}
\]
where the contaminated distribution becomes $F_\epsilon=(1-\epsilon)F+\epsilon \delta_{\rvx_0}$, where \( \delta_{\rvx_0} \) is the Dirac delta function centered at \( \rvx_0 \) and $F$ is the distribution of $\rvx$. Then, we have:
\[
IF(\rvx_0; T_{\ell_2}, F) =  \rvx_0 - \vy,
\] and 
\[
IF(\rvx_0; T_{\ell_1}, F) 
=\frac{   w_0 \left(\rvx_0-\rvz
\right)  }{ \sum_{d=1}^{D} w_d} \text{ where } w_0=\frac{1}{|\rvx_0-\vy|}.\]
\end{theorem}
\begin{proof}
    Please refer to Appendix~\ref{sec:proof_influecen_function}.
\end{proof}

Theorem~\ref{thm:influence_function} provide several insights into the robustness of both $\ell_2$ and $\ell_1$ models:
\begin{itemize}[left=0.0em]
    \item For the $\ell_2$-model, the influence function is given by $\rvx_0 - \vy$, indicating that the sensitivity of the $\ell_2$ model depends on the difference between the perturbation $\rvx_0$ and the clean estimate $\vy$.
    \item For the $\ell_1$-model, the influence function is $\frac{   w_0 \left(\rvx_0-\rvz \right)  }{ \sum_{d=1}^{D} w_d}$, where $w_0 = \frac{1}{|\rvx_0-\vy|}$. Although the robustness of the $\ell_1$ model is affected by the difference $\rvx_0-\rvz$, the influence can be significantly mitigated by the weight $w_0$, particularly when $\rvx_0$ deviates from the estimation $\vy$ of majority of the clean data.
\end{itemize}





\section{Robustness Reprogramming}
\label{sec:robustness_reprogramming}

% \xr{here we can introduce details on how to apply the robust feature mapping to any given model}

\xr{here, the most important thing is to motivate and justify the challenges and uniqueness of robustness reprogramming. Basically, we need to show it is novel and different from any existing works, and why it is useful in practice (for different paradigms)}



Many approaches have been proposed to enhance adversarial robustness, including robust training and regularization techniques~\citep{madry2017towards,cisse2017parseval,zheng2016improving}. However, these strategies inevitably fall into some pitfalls: (1) They often constrain weight properties to improve robustness, which disrupts feature pattern matching and results in a serious sacrifice of  natural performance. (2) Robust training methods heavily depend on the quality of augmented perturbations during training and are prone to overfitting. (3) These methods also suffer from significant forgetting issues, requiring retraining from scratch when exposed to new and different noisy environments, posing a significant efficiency challenge in the era of large-scale models. To address these issues, in this section, we propose a novel and flexible method, \emph{Robustness Reprogramming}, which can be applied across three paradigms to improve the robustness of any given deep learning model.



\begin{wrapfigure}{r}{0.51\textwidth}
\vspace{-0.8cm}
\begin{minipage}{0.48\textwidth}
\begin{algorithm}[H]
\caption{Hybrid Architecture}
\label{alg:hybird_arch}
\begin{algorithmic}

\Require  
$\{\rvx_d\}_{d=1}^D$, $\{\rva_d\}_{d=1}^D$, $\lambda$.

\State Initialize $\rvz^{(0)}_{\ell_1} = \rvz_{\ell_2}=\sum_{d=1}^D\rva_d\cdot\rvx_d$


\For{$k = 0, 1,\dots, K-1$}
\State $ w_d^{(k)} = \frac{1}{|\rva_d \rvx_d - \rvz^{(k)}_{\ell_1} / D|} \text{ for each } d \in [D]$ 
\State $\rvz^{(k+1)}_{\ell_1}
    =D\cdot \frac{\sum_{d=1}^D  w^{(k)}_d \rva_d\rvx_d}{\sum_{d=1}^D  w^{(k)}_d}$
    
\EndFor

\hspace{-0.8cm} \Return $\lambda \cdot \rvz_{\ell_2} + (1 - \lambda) \cdot \rvz^{(K)}_{\ell_1}$
\hspace{-3.8cm}
\end{algorithmic}
\end{algorithm}


\end{minipage}

\end{wrapfigure}


When considering the iterative $\ell_1$-model: $\rvz^{(k+1)} =D\cdot \frac{\sum_{d=1}^D w^{(k)}_d \rva_d\rvx_d}{\sum{d=1}^D w^{(k)}d}$, it is essentially a reweighted version of the vanilla $\ell_2$-model: $\rvz = \sum_{d=1}^D \rva_d \rvx_d$, which adaptively adjusts the original weights to mitigate the impact of potential outlying perturbed features. This architecture, unlike existing parameter modification methods~\citep{madry2017towards,cisse2017parseval,zheng2016improving}, largely preserves the feature pattern matching behaviors between the weight $\rva$ and the feature $\rvx$. This facilitates the reuse of the pretrained parameters from the $\ell_2$ model, either by plugging in the $\ell_1$-based architecture with pretrained parameters or performing minimal additional fine-tuning.
Especially in today's deep learning era with increasing model size, reusing pretrained parameters can significantly save time and resources, fostering the development of trustworthy AI in large-scale models.




While $\ell_1$-estimation enhances model robustness, it can lead to a decrease in clean accuracy, particularly in deeper models. This reduction in performance may be due to the increasing estimation error between $\ell_2$ and $\ell_1$ estimations across layers. To balance the trade-off between $\ell_1$ and $\ell_2$-based models, it is necessary to develop a hybrid architecture as in Algorithm~\ref{alg:hybird_arch}.
% $$
%     \rvz^{(0)}_{\ell_1} = \rvz_{\ell_2} = \sum_{d=1}^D \rva_d \rvx_d
% $$
% $$
%     \rvz^{(k+1)}_{\ell_1} = D \cdot \frac{\sum_{d=1}^D w^{(k)}_d \rva_d \rvx_d}{\sum_{d=1}^D w^{(k)}_d}, \quad \text{where } w_d^{(k)} = \frac{1}{|\rva_d \rvx_d - \rvz^{(k)}_{\ell_1} / D|}, \, k=0, \dots, K-1
% $$
% $$
%     \rvz = \lambda \cdot \rvz_{\ell_2} + (1 - \lambda) \cdot \rvz^{(K)}_{\ell_1}
% $$


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/paradigm.png}
    \caption{
    \emph{Robustness Reprogramming} with three paradigms: 1) Paradigm 1  freezes the model parameters and treats $\lambda$ as a fixed hyperparameter; 2) Paradigm 2 freezes the model parameters but allows $\lambda$ to be learnable; Paradigm 3 enables both the model parameters and $\lambda$ to be learnable.
    }
    \label{fig:three_paradigm}
\end{figure}

This hybrid can be flexibly employed under 3 paradigms as in Figure~\ref{fig:three_paradigm} according to the practice scenarios to enhance the resilience of any given backbone models:

\xr{do not use $\lambda$ in the name of your method/paradigm, it is strange since the notation can be any symbol. Maybe use parameter and hyperparameters (or other names, such as balance/trade-off) to distinguish them}

\textbf{Paradigm 1 (without fine-tuning, good robustness with zero cost).}
As deep learning models become increasingly larger, it is critical to fully utilize pretrained model parameters. Since the robust $\ell_1$ estimation slightly refines the vanilla $\ell_2$ estimation through an adaptive reweighting scheme, ensuring that the pretrained $\ell_2$ parameters still fit well within the $\ell_1$-based architecture. Experiments also validate that while the $\ell_1$-based architecture with $\ell_2$ parameters may slightly reduce natural performance, it significantly enhances robustness. Additionally, by adjusting the hyperparameter $\lambda$ with pretrained parameters, we can strike an ideal balance between natural and robust accuracy.
It is worth noting that relying solely on pretrained parameters with plug-and play paradigm significantly reduces computational costs, which is crucial in the era of large-scale deep learning.

\textbf{Paradigm 2 (only fine-tuning $\lambda$, strong robustness with slight cost.} One drawback of Paradigm 1 is that we specify the same $\lambda$ for all the layers and need to conduct brute force hyper-parameters search to obtain the optimal one. However, 
hyper-parameters search is time-consuming and labor-intensive. Moreover, different layers may need different $\lambda$ to balance the $\ell_2$ and $\ell_1$-models. To solve it, we propose Paradigm 2, which makes $\lambda$ learnable to automatically learn the optimal $\lambda$ combinations. This paradigm only finetune the $\lambda$ and keep the model parameters frozen, which is still efficient.

\textbf{Paradigm 3: (with fine-tuning, superior robustness with acceptable cost).}  
Although Paradigm 2 delivers excellent performance in most cases, it may fall short in deeper models, where the estimation bias between $\ell_2$ and $\ell_1$ estimators accumulates across layers. To address this, we make both the model parameters $\{\rva_d\}_{d=1}^D$ and the weight $\lambda$ learnable. By refining these parameters based on the pretrained model, we can prevent clean performance degradation. Moreover, with a learnable $\lambda$ during adversarial training, the model can automatically select the optimal combination to enhance both clean and robust performance.

\xr{I understand you describe some details about motivation here. It is better to also have a short and high-level motivation at the beginning to motivate why we propose three paradigms.}

\xr{In general, when we write paper, we need to make the life of reviewers easy. Even if they do not read many of your detailed descriptions, they know why and what you are doing by reading the beginning of your section/subsection/paragraphs}


\textbf{Advantages.} (1) \emph{Flexibility.} Our proposed \emph{Robustness Reprogramming} can be flexibly applied under 3 paradigms for the consideration of practice resource constraints and robustness requirements.
(2) \emph{Reliability.} Our method can achieve excellent robustness while maintaining decent natural performance.
(3) \emph{Compatibility.} Our method largely maintain the feature pattern matching behaviors of vanilla backbone models, making it highly compatible with  pretrained parameters of $\ell_2$-model and the hybrid architecture.





==> section/reprogram.tex <==
\section{Robustness Reprogramming}
\label{sec:robustness_reprogramming}

\xr{I think in this section we do not need to talk about existing works. just focus on our goal on robustness reprogramming. The major motivation and challenge is to balance the tradeoff between robustness and accuracy}

% \xr{here we can introduce details on how to apply the robust feature mapping to any given model}

% \xr{here, the most important thing is to motivate and justify the challenges and uniqueness of robustness reprogramming. Basically, we need to show it is novel and different from any existing works, and why it is useful in practice (for different paradigms)}



% Many approaches have been proposed to enhance adversarial robustness, including robust training and regularization techniques~\citep{madry2017towards,cisse2017parseval,zheng2016improving}. 

% Robust training and regularization techniques
Robust and regularized training techniques~\citep{madry2017towards,cisse2017parseval,zheng2016improving} 
% have been shown to be the 
are the most reliable approaches to enhance adversarial robustness~\citep{croce2020robustbench}.
% through costly training of model parameters.
However, these strategies face several limitations:
% inevitably fall into some pitfalls: 
(1) They constrain model parameters
% weight properties
to improve robustness, which disrupts feature pattern matching and could result in a serious sacrifice of  natural performance; (2) Robust training methods heavily depend on the quality of augmented perturbations during training and are prone to overfitting; and (3) These methods also suffer from significant forgetting issues, requiring retraining from scratch when exposed to new and different noisy environments, posing a significant efficiency challenge in the era of large-scale models. To address these issues, 
% in this section, 
built upon the technique in Section~\ref{sec:represenation_learning},
we propose a transformative method, \emph{Robustness Reprogramming} 
% which can be applied across  
to improve the robustness of any given deep learning models through three flexible paradigms. \xr{this part needs to be rephrased. Our goal is not to address the limitations of them, but provide a new perspective for improvements}



\begin{wrapfigure}{r}{0.51\textwidth}
\vspace{-0.8cm}
\begin{minipage}{0.50\textwidth}
\begin{algorithm}[H]
% \caption{Hybrid Architecture}
\caption{Robustness Reprogramming}
\label{alg:hybird_arch}
\begin{algorithmic}

\Require  
$\{x_d\}_{d=1}^D$, $\{a_d\}_{d=1}^D$, $\lambda$.

\State Initialize $z^{(0)}_{NRPM} = z_{LPM}=\sum_{d=1}^D a_d\cdot x_d$


\For{$k = 0, 1,\dots, K-1$}
\State $ w_d^{(k)} = \frac{1}{|a_d x_d - z^{(k)}_{NRPM} / D|} \text{ for each } d \in [D]$ 
\State $z^{(k+1)}_{NRPM}
    =D\cdot \frac{\sum_{d=1}^D  w^{(k)}_d a_dx_d}{\sum_{d=1}^D  w^{(k)}_d}$
    
\EndFor

\hspace{-0.8cm} \Return $\lambda \cdot z_{LPM} + (1 - \lambda) \cdot z^{(K)}_{NRPM}$
\hspace{-3.8cm}
\end{algorithmic}
\end{algorithm}


\end{minipage}

\vspace{-0.25in}
\end{wrapfigure}


When considering the iterative NRPM: $z^{(k+1)} =D\cdot \frac{\sum_{d=1}^D w^{(k)}_d a_dx_d}{\sum{d=1}^D w^{(k)}_d}$, it is essentially a reweighted version of the vanilla LPM: $z = \sum_{d=1}^D a_d x_d$, which adaptively adjusts the original weights to mitigate the impact of potential outlying perturbed features. This architecture, unlike existing parameter modification methods~\citep{madry2017towards,cisse2017parseval,zheng2016improving}, largely preserves the feature pattern matching behaviors between the weight $a$ and the feature $x$. This facilitates the reuse of the pretrained parameters from LPM, either by plugging in NRPM architecture with pretrained parameters or performing minimal additional fine-tuning.
Especially in today's deep learning era with increasing model size, reusing pretrained parameters can significantly save time and resources, fostering the development of trustworthy AI in large-scale models.




While NRPM enhances model robustness, it can lead to a decrease in clean accuracy, particularly in deeper models. This reduction in performance may be due to the increasing estimation error between OLS and LDA estimations across layers. To balance the trade-off between LPM and NRPM, it is necessary to develop a hybrid architecture as in Algorithm~\ref{alg:hybird_arch}.
% $$
%     z^{(0)}_{NRPM} = z_{LPM} = \sum_{d=1}^D a_d x_d
% $$
% $$
%     z^{(k+1)}_{NRPM} = D \cdot \frac{\sum_{d=1}^D w^{(k)}_d a_d x_d}{\sum_{d=1}^D w^{(k)}_d}, \quad \text{where } w_d^{(k)} = \frac{1}{|a_d x_d - z^{(k)}_{NRPM} / D|}, \, k=0, \dots, K-1
% $$
% $$
%     z = \lambda \cdot z_{LPM} + (1 - \lambda) \cdot z^{(K)}_{NRPM}
% $$

% \vspace{-0.2in}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/paradigm.png}
    \vspace{-0.1in}
    \caption{
    \emph{Robustness Reprogramming} with three paradigms: 1) Paradigm 1  freezes the model parameters and treats $\lambda$ as a fixed hyperparameter; 2) Paradigm 2 freezes the model parameters but allows $\lambda$ to be learnable; Paradigm 3 enables both the model parameters and $\lambda$ to be learnable.
    }
    \label{fig:three_paradigm}
    \vspace{-0.2in}
\end{figure}

This hybrid can be flexibly employed under 3 paradigms as in Figure~\ref{fig:three_paradigm} according to the practice scenarios to enhance the resilience of any given backbone models:

% \xr{do not use $\lambda$ in \lambdthe name of your method/paradigm, it is strange since the notation can be any symbol. Maybe use parameter and hyperparameters (or other names, such as balance/trade-off) to distinguish them}

\textbf{Paradigm 1: without fine-tuning, good robustness with zero cost.}
As deep learning models become increasingly larger, it is critical to fully utilize pretrained model parameters. Since the robust NRPM slightly refines the vanilla LPM through an adaptive reweighting scheme, ensuring that the pretrained LPM parameters still fit well within NRPM architecture. Experiments also validate that while NRPM architecture with LPM parameters only slightly reduce natural performance, it significantly enhances robustness. Additionally, by adjusting the hyperparameter $\lambda$ with pretrained parameters, we can strike an ideal balance between natural and robust accuracy.
It is worth noting that relying solely on pretrained parameters with plug-and play paradigm significantly reduces computational costs, which is crucial in the era of large-scale deep learning.

\textbf{Paradigm 2: only fine-tuning $\lambda$, strong robustness with slight cost.} One drawback of Paradigm 1 is that we specify the same $\lambda$ for all the layers and need to conduct brute force hyper-parameters search to obtain the optimal one. However, 
hyper-parameters search is time-consuming and labor-intensive. Moreover, different layers may need different $\lambda$ to balance the LPM and NRPMs. To solve it, we propose Paradigm 2, which makes $\lambda$ learnable to automatically learn the optimal $\lambda$ combinations. This paradigm only finetune the $\lambda$ and keep the model parameters frozen, which is still efficient.

\textbf{Paradigm 3: with fine-tuning, superior robustness with acceptable cost.}  
Although Paradigm 2 delivers excellent performance in most cases, it may fall short in deeper models, where the estimation bias between LPM and NRLPM estimators accumulates across layers. To address this, we make both the model parameters $\{a_d\}_{d=1}^D$ and the weight $\lambda$ learnable. By refining these parameters based on the pretrained model, we can prevent clean performance degradation. Moreover, with a learnable $\lambda$ during adversarial training, the model can automatically select the optimal combination to enhance both clean and robust performance.

% \xr{I understand you describe some details about motivation here. It is better to also have a short and high-level motivation at the beginning to motivate why we propose three paradigms.}

% \xr{In general, when we write paper, we need to make the life of reviewers easy. Even if they do not read many of your detailed descriptions, they know why and what you are doing by reading the beginning of your section/subsection/paragraphs}


\textbf{Advantages.} (1) \emph{Flexibility.} Our proposed \emph{Robustness Reprogramming} can be flexibly applied under 3 paradigms for the consideration of practice resource constraints and robustness requirements.
(2) \emph{Reliability.} Our method can achieve excellent robustness while maintaining decent natural performance.
(3) \emph{Compatibility.} Our method largely maintain the feature pattern matching behaviors of vanilla backbone models, making it highly compatible with  pretrained parameters of LPM and the hybrid architecture.





==> section/statement.tex <==
\section*{Statement} 
\textbf{Ethics statement.} 
This paper proposes robustness reprogramming techniques to enhance the robustness and safety of machine learning models. We do not identify any potential negative concerns.
\textbf{Reproducibility statement.} 
This paper provides all necessary technique details for reproducibility, including theoretical analysis, algorithm details, experimental settings, pseudo code, implementation, and source code of the proposed techniques.

